A Closer Look at Geometric Temporal Dynamics for Face Anti-Spoofing

Face anti-spoofing (FAS) is indispensable for a face recognition system. Many texture-driven countermeasures were developed against presentation attacks (PAs), but the performance against unseen domains or unseen spoofing types is still unsatisfactory. Instead of exhaustively collecting all the spoofing variations and making binary decisions of live/spoof, we offer a new perspective on the FAS task to distinguish between normal and abnormal movements of live and spoof presentations. We propose Geometry-Aware Interaction Network (GAIN), which exploits dense facial landmarks with spatio-temporal graph convolutional network (ST-GCN) to establish a more interpretable and modularized FAS model. Additionally, with our cross-attention feature interaction mechanism, GAIN can be easily integrated with other existing methods to significantly boost performance. Our approach achieves state-of-the-art performance in the standard intra- and cross-dataset evaluations. Moreover, our model outperforms state-of-the-art methods by a large margin in the cross-dataset cross-type protocol on CASIA-SURF 3DMask (+10.26% higher AUC score), exhibiting strong robustness against domain shifts and unseen spoofing types.

==> tables/fusion_cross.tex <==
\begin{table}[t]
    \begin{center}
    \scalebox{0.75}{\begin{tabularx}{0.8\columnwidth}{cc *2{Y}}
        \toprule
        & & \multicolumn{2}{c}{O\&C\&I to M} \\
        \cmidrule(l){3-4}
        Attn & \# of Cls & HTER(\%) & AUC(\%) \\
        \midrule
        \multicolumn{2}{c}{Baseline} & 7.38 & 96.97 \\
        \midrule
        \xmark & 2 & 7.14 & 97.47 \\
        \xmark & 3 & 4.29 & 98.76 \\
        \cmark & 3 & \textbf{4.05} & \textbf{98.92} \\
        \bottomrule
    \end{tabularx}}
    \end{center}
    \caption{Ablation study of the feature interaction strategy under the cross-dataset (O\&C\&I to M) setting. Note: \textit{Attn} indicates whether cross-attention is adopted in the method; \textit{\# of Cls} indicates if common live/spoof binary classification or the proposed 3-class classification is performed.}
    \label{tab:fusion_cross}
\end{table}

% \begin{table*}[t]
%     \begin{center}
%     \scalebox{0.9}{\begin{tabularx}{1\textwidth}{cc *8{Y}}
%         \toprule
%         & & \multicolumn{2}{c}{O\&C\&I to M} & \multicolumn{2}{c}{O\&M\&I to C} & \multicolumn{2}{c}{O\&C\&M to I} & \multicolumn{2}{c}{I\&C\&M to O} \\
%         \cmidrule(l){3-4} \cmidrule(l){5-6} \cmidrule(l){7-8} \cmidrule(l){9-10}
%         attn(?) & cls(?) & HTER(\%) & AUC(\%) & HTER(\%) & AUC(\%) & HTER(\%) & AUC(\%) & HTER(\%) & AUC(\%) \\
%         \midrule
%         \multicolumn{2}{c}{Baseline} & 7.38 & 96.97 & 9.89 & 95.28 & 12.29 & 94.49 & 14.03 & 93.07 \\
%         \midrule
%         \xmark & 2 & 7.38 & 97.50 & 10.56 & 95.31 & 11.43 & 94.47 & 13.18 & 94.39 \\
%         \xmark & 3 & 4.29 & 98.76 & 8.52 & 96.04 & 8.57 & 97.08 & 12.40 & 95.04 \\
%         \cmark & 3 & 4.05 & 98.92 & 8.52 & 96.02 & 8.50 & 97.27 & 12.50 & 95.12 \\
%         \bottomrule
%     \end{tabularx}}
%     \end{center}
%     \caption{Caption}
%     \label{tab:fusion_cross}
% \end{table*}

==> tables/gcn_alone.tex <==
\begin{table}[t]
    \begin{center}
    \scalebox{0.75}{\begin{tabularx}{0.8\columnwidth}{cc *2{Y}}
        \toprule
        & & \multicolumn{2}{c}{O\&C\&I to M} \\
        \cmidrule(l){3-4}
         &  & HTER(\%) & AUC(\%) \\
        \midrule
        \multicolumn{2}{c}{Baseline} & 7.38 & 96.97 \\
        \midrule
        \multicolumn{2}{c}{ST-GCN-3cls} & 35.95 & 65.92 \\
        \multicolumn{2}{c}{Baseline + \textbf{GAIN}} & \textbf{4.05} & \textbf{98.92} \\
        \bottomrule
    \end{tabularx}}
    \end{center}
    \caption{Ablation study of the performance of proposed ST-GCN alone under the cross-dataset (O\&C\&I to M) setting.}
    \label{tab:gcn_alone}
\end{table}
